PIER: A Novel Metric for Evaluating What Matters in Code-Switching

Code-switching, the alternation of languages within a single discourse, presents a significant challenge for Automatic Speech Recognition. Despite the unique nature of the task, performance is commonly measured with established metrics such as Word-Error-Rate (WER). However, in this paper, we question whether these general metrics accurately assess performance on code-switching. Specifically, using both Connectionist-Temporal-Classification and Encoder-Decoder models, we show fine-tuning on non-code-switched data from both matrix and embedded language improves classical metrics on code-switching test sets, although actual code-switched words worsen (as expected). Therefore, we propose Point-of-Interest Error Rate (PIER), a variant of WER that focuses only on specific words of interest. We instantiate PIER on code-switched utterances and show that this more accurately describes the code-switching performance, showing huge room for improvement in future work. This focused evaluation allows for a more precise assessment of model performance, particularly in challenging aspects such as inter-word and intra-word code-switching.

==> graphs/w-small-eval.tex <==
\begin{tikzpicture}
    \begin{axis}[
    %xlabel={Model Type},
    ylabel={Performance Metric (\%)},
    legend style={
        at={(1,1.15)},
        anchor=south east,
        legend columns=2,
        font=\footnotesize, % Change font size of legend
        cells={anchor=west}, % Adjust cell alignment
        /tikz/legend image code/.code={%
            \draw [line width=0.8pt] (0,0.5ex) -- (0.5ex,0.5ex); % Adjust line thickness in legend
        },
    },
    xtick={1,2},
    xticklabels={Base Model, Fine-tuned Model},
    tick label style={font=\scriptsize}, % Change font size of tick labels
    grid=major,
    width=0.9\linewidth, % Adjust width to fit within one column
    height=0.6\linewidth, % Adjust height proportionally
    ]
        % Fisher data for W-small
        \addplot[
            color=blue,
            mark=square,
            line width=0.8pt,
            ]
            coordinates {(1,35.98) (2,36.77)};
        \addplot[
            color=blue,
            dashed,
            mark=square,
            line width=0.8pt,
            ]
            coordinates {(1,48.14) (2,63.52)};
        
        % ARZEN data for W-small
        \addplot[
            color=red,
            mark=triangle,
            line width=0.8pt,
            ]
            coordinates {(1,69.16) (2,55.08)};
        \addplot[
            color=red,
            dashed,
            mark=triangle,
            line width=0.8pt,
            ]
            coordinates {(1,75.91) (2,78.10)};
        
        % SEAME.MAN data for W-small
        \addplot[
            color=green,
            mark=o,
            ]
            coordinates {(1,41.17) (2,42.09)};
        \addplot[
            color=green,
            dashed,
            mark=o,
            line width=0.8pt,
            ]
            coordinates {(1,74.95) (2,88.82)};
        
        % SEAME.SGE data for W-small
        \addplot[
            color=orange,
            mark=star,
            line width=0.8pt,
            ]
            coordinates {(1,68.24) (2,87.67)};
        \addplot[
            color=orange,
            dashed,
            mark=star,
            line width=0.8pt,
            ]
            coordinates {(1,83.08) (2,97.60)};
        
        % Adding legend entries
       % \addlegendentry{Fisher WER}
       % \addlegendentry{Fisher PER}
       % \addlegendentry{ARZEN WER}
       % \addlegendentry{ARZEN PER}
       % \addlegendentry{SEAME.MAN WER}
       % \addlegendentry{SEAME.MAN PER}
       % \addlegendentry{SEAME.SGE WER}
       % \addlegendentry{SEAME.SGE PER}

    \end{axis}
\end{tikzpicture}
